Answering the "why" in Answer Set Programming - A Survey of Explanation Approaches

Artificial Intelligence (AI) approaches to problem-solving and decision-making are becoming more and more complex, leading to a decrease in the understandability of solutions. The European Union's new General Data Protection Regulation tries to tackle this problem by stipulating a "right to explanation" for decisions made by AI systems. One of the AI paradigms that may be affected by this new regulation is Answer Set Programming (ASP). Thanks to the emergence of efficient solvers, ASP has recently been used for problem-solving in a variety of domains, including medicine, cryptography, and biology. To ensure the successful application of ASP as a problem-solving paradigm in the future, explanations of ASP solutions are crucial. In this survey, we give an overview of approaches that provide an answer to the question of why an answer set is a solution to a given problem, notably off-line justifications, causal graphs, argumentative explanations and why-not provenance, and highlight their similarities and differences. Moreover, we review methods explaining why a set of literals is not an answer set or why no solution exists at all.

==> discussion.tex <==
%!TEX root = justificationSurvey.tex
\vspace{2cm}
\section{Discussion}
\label{sec:discussion}

\CHANGED
This section gives an overview of differences and similarities of the ASP explanation approaches 
reviewed in this paper
and study some of the general problems faced by these approaches.
% We furthermore discuss related approaches, e.g. further methods for explaining logic programming solutions as well as visualisations of logic programs.
\END
%\citeNS{Lifschitz10} listed thirteen different definitions of the concept of answer set (and pointed out that even more exist).
%These definitions are equivalent to each other (at least for normal programs), but provide alternative pictures of the intuitive meaning of logic programs or lead to different algorithms for generating answer sets.
%In this sense, it is not surprising that there exist several ways of explaining the solutions to consistent programs and the errors in inconsistent ones.
%%answering why some conclusion has been reached with respect to some logic program.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}
 \caption{Comparison of explanation approaches for consistent logic programs under the answer set semantics.}
 \label{tab:comparison:explanation}
 \begin{tabular}{ l l l l l } 
  \multirow{2}{2.5cm}{\textbf{approach}} & \multirow{2}{2cm}{\textbf{logic program}} & \multirow{2}{2cm}{\textbf{explanation in terms of}} & \multirow{2}{1.5cm}{\textbf{derivation steps included}} & \multirow{2}{2cm}{\textbf{explains}} \\ \\ \\
  \hline
  \multirow{2}{2.5cm}{off-line justifications} & normal LP & \multirow{2}{2.5cm}{literal dependency} & all & \multirow{2}{2cm}{one literal (not) in answer set} \\ \\ \\
  \hline
  \multirow{2}{2.5cm}{LABAS justifications} & \multirow{2}{2cm}{normal extended LP} & \multirow{2}{2.5cm}{literal dependency} & some & \multirow{2}{2cm}{one literal (not) in answer set} \\ \\ \\
  \hline
  \multirow{2}{2.5cm}{causal justifications} &
  \multirow{2}{2.5cm}{extended LP with nested expressions in the body}
   & \multirow{2}{2.5cm}{rule-literal dependency} & all & \multirow{2}{2cm}{one literal in answer set} \\ \\ \\ \\
  \hline
  \multirow{2}{2.5cm}{extended causal justifications} & \multirow{2}{2cm}{normal extended LP} & \multirow{2}{2.5cm}{rule-literal dependency} & all &\multirow{2}{2cm}{one literal (not) in answer set}\\ \\ \\
  \hline
  \multirow{2}{2.5cm}{rule-based justifications} & normal LP & \multirow{2}{2cm}{rule dependency} & all & \multirow{2}{2cm}{one literal (not) in answer set}\\ \\ \\
  \hline
  \multirow{2}{2.5cm}{why-not provenance} & normal LP & \multirow{2}{2cm}{rule dependency} & all & \multirow{2}{2cm}{one literal (not) in the complete well-founded model\footnotemark} \\ \\ \\ \\ \\
  \hline
  formal theory & normal LP & \multirow{2}{2cm}{literal dependency} & all & \multirow{2}{2cm}{the whole answer set}\\ \\
  \hline
 \end{tabular}
 \end{table}


 


 \begin{table}
 \caption{Comparison of explanation approaches for consistent logic programs under the answer set semantics (continued).}
 \label{tab:comparison:explanation2}
 \begin{tabular}{ l l l l l } 
  %\hline
  \multirow{2}{2.5cm}{\textbf{approach}} & \multirow{2}{2cm}{\textbf{computation uses other models}} & \multirow{2}{2cm}{\textbf{explanation of negative literals}} & \multirow{2}{2cm}{\textbf{infinite explanations}} & \multirow{2}{2cm}{\textbf{infinitely many explanations}} \\ \\ \\
  \hline
  \multirow{2}{2.5cm}{off-line justifications} & \multirow{2}{2cm}{well-founded model} & \multirow{2}{2cm}{assumed or further explained} & \multirow{2}{2cm}{no, if the program is finite} & \multirow{2}{2cm}{no, if the program is finite}\\ \\ \\
  \hline
  \multirow{2}{2.5cm}{LABAS justifications} & no & \multirow{2}{2cm}{further explained} & yes & yes\\ \\
  \hline
  \multirow{2}{2.5cm}{causal justifications} & no & assumed & no & \multirow{2}{2cm}{no, if the program is finite}\\ \\ \\
  \hline
  \multirow{2}{2.5cm}{extended causal justifications} & \multirow{2}{2cm}{well-founded model}  & \multirow{2}{2cm}{assumed or further explained} & \multirow{2}{2cm}{no, if the program is finite} & \multirow{2}{2cm}{no, if the program is finite}\\ \\ \\
  \hline
  \multirow{2}{2.5cm}{rule-based justifications} & no  & \multirow{2}{2cm}{further explained} &  \multirow{2}{2cm}{no, if the program is finite} &  \multirow{2}{2cm}{no, if the program is finite} \\ \\ \\
  \hline
  \multirow{2}{2.5cm}{why-not provenance} &  \multirow{2}{2cm}{(do not need answer sets)} & \multirow{2}{2cm}{further explained} & \multirow{2}{2cm}{no, if the program is finite} & \multirow{2}{2cm}{no, if the program is finite}\\ \\ \\ \\
  \hline
  formal theory & no  & \multirow{2}{2cm}{further explained} & yes &  \multirow{2}{2cm}{no, if the program is finite} \\ \\ \\
  \hline
 \end{tabular}
 \end{table}
 % \comment{I think that I do not understood correctly what the ``dependency on other models column'' means?}
 % \reply{I meant that e.g. to compute off-line justifications you don't just need the answer set being justified, but also the well-founded model (if I understand it correctly) in order to compute the assumptions. In contrast, in LABAS justifications, you only need the answer set.}
 % \comment{Does it make more sense to have exponential blow-up in the table rather than infinity?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Justification Approaches}
In Sections~\ref{sec:offline} to~\ref{sec:other_justifications} we surveyed the most prominent approaches for justifying the solutions to consistent logic programs under the answer set semantics.
Note that throughout these sections, by referencing an answer set to justify, we implicitly assumed that logic programs are consistent.
While explaining the justification approaches, we already pointed out differences and similarities between these approaches.
Some of these are reiterated in Tables~\ref{tab:comparison:explanation} and~\ref{tab:comparison:explanation2}, which provide a comparative overview of various features of the justification approaches.
\CHANGED
In particular, Table~\ref{tab:comparison:explanation} illustrates for which types of logic programs the different justification approaches are defined, in which terms they explain answer sets (i.e. dependencies between rules or literals), whether all parts of a literal's derivation are included in a justification, and what precisely is being explained, i.e. a literal in an answer set, a literal not contained in an answer set, or a whole answer set.
%
%
\footnotetext{\CHANGED The why-not provenance corresponding to each answer set can then be obtained by forcing the atoms not in the answer set as assumptions, similalr as how it has been done with extended causal justifications.}
%
%
Table~\ref{tab:comparison:explanation} complements this comparison, by showing whether justification approaches make use of logic programming models other than the answer set in question when constructing a justification, whether negative literals occur in justifications and, if so, how their truth value is explained, whether justifications may be infinite, and whether there may be infinitely many justifications.
\END
In the following, we discuss some of the differences between the justification approaches in more detail and highlight some of their advantages and disadvantages.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Explanatory Elements}
Due to the usage of different definitions of answer set, the different justifications embody distinct ideas. 
For instance, the intuition of \mbox{off-line} justifications (Section~\ref{sec:offline}) can be traced back to Prolog tabled justifications~\cite{roychoudhuryRR00};
% \cite{Specht93,PemmasaniGDRR03};
LABAS justifications (Section~\ref{sec:labas}) have an argumentative flavour and are based on a correspondence between logic programs and their translation into argumentation frameworks \cite{SchulzT2015,SchulzT2016};
while causal justifications (Section~\ref{sec:causal}) rely on a causal interpretation of rules and the idea of causal chain~\cite{lewis1973causation}.
Despite their differences, these three approaches share the fact that they explain why a literal belongs to some answer set using a ``concise'' graph structure (in the sense that these graphs do not contain information not related to the literal in question).

The \mbox{why-not} provenance (Section~\ref{sec:why-not}), which is based on the concept of provenance inherited from the database literature~\cite{GreenKT07}, also shares with these approaches the idea of building concise justifications for each literal.
However, why-not provenance justifications are set based (instead of graph based) and are built without referring 
to a specific answer set, so justifications are answer set independent.
%independently to each answer set.
\CHANGED
On the other hand, the justifications for a particular answer set can be obtained by ``forcing'' the appropriate assumptions as done in extended causal justifications.
\END

A similar point of view is also shared by rule-based justifications (Section~\ref{sec:rule-based}), which are based on the concept of an \emph{\mbox{\tt ASPeRiX} computation}~\cite{LefevreBSG17}.
Conceptually, the major difference between this and the previously mentioned approaches lies in what is considered as assumptions,
i.e. as elements that do not need to be further justified:
rules in the case of rule-based justifications and literals in the case of the other approaches.


%\footnotetext{In this survey, we have limited ourselves to normal extended logic programs. For a the definition of causal justifications for programs with nested expressions in the body, we refer to~\cite{Fandinno16}.}
% \sidecomment{Don't forget to place the footnote \reply{Also add the same to the last subsection}}


The formal theory of justifications~(Section~\ref{sec:formal})
aims to explain the differences between different logic programming semantics by identifying how their conclusions are justified.
Contrary to the other approaches, it provides justifications for a whole answer set instead of concise justifications for each literal.
This is similar to debugging systems 
(Section~\ref{sec:debugging}), which explain why a whole set of literals is not an answer set, rather than explaining a specific literal.
%like \spock~(Section~\ref{sec:debugging:spock})
%and \dwasp~(Section~\ref{sec:debugging:dwasp}),
%which are respectively based on unfounded set based definition of answer sets~\cite{LinZ2004,Lee2005} and the idea of an unsatisfiable core~\cite{AlvianoDFLR2013,AlvianoDLR15}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The Problem of Exponentially Many Justifications}


As mentioned in the introduction, a key point for a human-understandable answer to the question why some conclusion is reached is its conciseness. 
Most justification approaches reviewed here have tackled this issue and provide justifications that only contain information related to the literal in question.
\CHANGED
However, a second issue is how many of these justifications there are.
In this section we show that the number of justifications is in general exponential \wrt\ the size of the program.
Let us start by continuing here the discussion about the light bulb scenario introduced in Example~\ref{ex:light} (page~\pageref{ex:light}).
\END



\input{switch}





Despite the fact that understanding negation-as-failure as a default allows to exponentially reduce the number of justifications on some knowledge representation scenarios as illustrated by the above example, there still exist logic programs that require an exponential number of justifications:

 % \comment{I made some changes here since we already showed that LABAS justifications suffer from exponential explosion.}

\vspace{2cm}

\begin{example}\label{ex:exponential}
\label{ex:exp}
Consider the following logic program adapted from~\cite{CabalarFF14}:
\begin{gather*}
\begin{IEEEeqnarraybox}[][t]{lCl"l}
p_1 & \leftarrow q_1
\\
p_1 & \leftarrow u_1
\end{IEEEeqnarraybox}
\hspace{1cm}
\begin{IEEEeqnarraybox}[][t]{lCl"l}
% p_1	& \leftarrow q_1
% \\
% p_1	& \leftarrow u_1
% \\
p_{i}		& \leftarrow &	p_{i-1} \wedge q_{i}
						&	\text{for }  i\in\set{2,\dotsc,n}
\\
p_{i}		& \leftarrow &	p_{i-1} \wedge u_{i}
						&	\text{for }  i\in\set{2,\dotsc,n}
\\
q_{i} && &  \text{for }  i\in\set{1,\dotsc,n}
\\
u_{i} && &  \text{for }  i\in\set{1,\dotsc,n}
\end{IEEEeqnarraybox}
\end{gather*}
and whose unique answer set is $\set{p_1,q_1,u_1\dotsc,p_n,q_n,u_n}$.
Note that $p_1$ can be justified using the facts~$q_0$ or~$u_0$;
the atom $p_2$ can be justified using the sets of facts $\set{q_1,q_2}$,
$\set{q_1,u_2}$, $\set{u_1,q_2}$ or $\set{u_1,u_2}$; and so on.
It is easy to see that atom~$p_n$ can be justified using $2^n$ different sets of facts and, thus, that the number of justifications grows exponentially with respect to the size of the program.
\qed
\end{example}


Although, this logic program has no deeper knowledge representation meaning, it points out a potential problem regarding the human-readability of the answers provided by current justification approaches.
\CHANGED
Note that the need of an exponential number of justifications illustrated by Example~\ref{ex:exponential} holds 
for any justification approach that records minimal sets of facts
used to derive the justified atom.
This does not mean that other kind of polynomial justifications can be used.
For instance,
for causal justifications or why-not provenance, a non-simplified formula could be
returned, and in this case the justification would be polynomial.
In our running example, we would have that $p_n$ is justified by the causal term
$(q_1 + u_1) * (q_2 + u_2) * \dotsc *  (q_n + u_n)$
or the why-not provenance formula
$(q_1 \vee u_1 \vee \neg not(p_1)) \wedge (q_2 \vee u_2 \vee \neg not(p_2)) \wedge \dotsc \wedge (q_n \vee u_n \vee \neg not(p_n))$.
On the other hand, these non-simplified expressions are not minimal and, thus, they not completely satisfy the concise criterion.
Another alternative is to provide simplified justification, by selecting only some of them in base a some imposed preferences~\cite{CabalarFF14}.
\END
For instance, approaches in databases~\cite{Specht93} and Prolog~\cite{roychoudhuryRR00} implicitly impose such preferences by selecting only the first negative literal of a rule that fails as its unique justification.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{negation-as-failure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Application-Oriented Considerations}
Our comparison so far has concentrated on the theoretical, or even philosophical, nature of justification approaches.
Another important, and distinguishing, aspect of justification approaches is their applicability when solving real-world problems.
In such situations, various challenges arise.

Firstly, representing a real-world problem may result in a large logic program, where literals may have long derivations, i.e. their truth value depends on a large number of rules.
It is then not clear, which information a justification should comprise in order to be, on the one hand, succinct enough for humans to understand, but,
% on the other hand provide, provide all important information.
on the other hand, complete enough to provide all important information.
For example, justification approaches where all derivation steps are included in the justification, that is all approaches other than LABAS justifications, may struggle with the succinctness when explaining a large logic program, as explanations grow with longer derivations.
In contrast, LABAS justifications are independent of the derivation length. However, a large logic \changed{program} may also comprise more dependencies on negative literals, thus increasing the size of LABAS justifications.
% The definition of causal justifications for normal programs~\cite{CabalarFF2014} allow to leave some rules unlabelled so that they are not recorded in justifications.
% However, combining this feature with disjunctive rules is still an open question.
More generally, it is an open problem how to effectively deal with the growing size (as well as the previously mentioned exponential number) of justifications.

In order to use justifications in real-world problems, they need to be automatically constructed.
Currently, only LABAS, causal and why-not provenance justifications have been implemented in working prototypes.\footnote{There also used to be an implementation of off-line justifications \cite{El-KhatibPS2005}, but this is not available anymore.}
A related issue is which type of logic programs can be explained. In practice, logic programs are rarely normal and often use additional language constructs, such as weight constraints and aggregates.
The only approach able to handle non-normal logic programs, i.e. logic programs with disjunctive heads, is the causal justification approach, which can also deal with nested expressions in the body.\footnote{In this survey, we have limited ourselves to normal extended logic programs. For a the definition of causal justifications for logic programs with nested expressions in the body, we refer to~\cite{Fandinno16}.}
Choice rules are handled by off-line justifications and in a limited way by causal justifications~\cite{CabalarF16}.
Note that explanations of additional language constructs have not been investigated so~far.

As a last challenge, we mention variables. Even though the theory of most justification approaches can easily be applied to programs with variables by considering the complete grounding of the program, it is questionable if this method yields meaningful justifications in practice.
The difficulty of handling variables in explanations of inconsistent programs is a further indication that justifications involving variables are non-trivial, and therefore an interesting consideration for future work.
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Debugging Approaches}
 In Section~\ref{sec:debugging}, we outlined the most prominent approaches to ASP debugging, i.e. the explanation of non-answer sets and inconsistency in logic programs.
 We have seen that these approaches follow different ideas as to what an explanation should encompass and that they use different methodologies to achieve this.
 Tables~\ref{tab:comparison:debugging} and~\ref{tab:comparison:debugging2} provide a comparative overview of the differences and similarities of the surveyed debugging approaches.
 \changed{In particular, Table~\ref{tab:comparison:debugging} compares debugging approaches concerning the type of logic programs that can be debugged, whether or not logic programs with variables as well as with language constructs such as aggregates or arithmetic terms can be debugged, and whether the approach can also be used to explain consistent logic programs.
 Table~\ref{tab:comparison:debugging2} complements this by illustrating whether the debugging approaches assume an intended answer set, or rather, whether they detect mistakes with respect to potentially intended answer sets, which types of errors in a logic program the debugging approaches distinguish, and whether the user can or has to interact with the debugger.}
 In the following, we discuss some of the distinguishing features in more detail so as to facilitate users to choose the appropriate debugging approach for their application.
 
  
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}
  \caption{Comparison of explanation approaches for inconsistent logic programs.}
 \label{tab:comparison:debugging}

 \begin{tabular}{ l l l l l} 
  \multirow{2}{2.5cm}{\textbf{approach}} & \multirow{2}{2cm}{\textbf{logic program}} & \multirow{2}{2cm}{\textbf{variables supported}} & \multirow{2}{2.5cm}{\textbf{additional language constructs}} & \multirow{2}{2cm}{\textbf{explain consistent LPs}} \\\\ \\
  \hline
  \multirow{2}{2.5cm}{\spock\ transformation 1} & normal LP & no & no & yes \\ \\
  \hline 
  \multirow{2}{2.5cm}{\spock\ transformation 2} & LP & no & no & \multirow{2}{2cm}{only non answer sets}\\ \\
  \hline
  \ouroboros & extended LP & yes & \multirow{2}{2.5cm}{arithmetic, comparison} & \multirow{2}{2cm}{only non answer sets}\\ \\
  \hline
  interactive \spock & LP & no & no & \multirow{2}{2cm}{only non answer sets}\\ \\
  \hline
  \dwasp & LP & yes & no & no\\
  \hline
  \stepping & extended LP & yes & \multirow{2}{2.5cm}{aggregates, weight constraints, external atoms} & yes \\ \\ \\ \\
  \hline
 \end{tabular}
 \end{table}

 
 \begin{table}
  \caption{Comparison of explanation approaches for inconsistent logic programs (continued).}
 \label{tab:comparison:debugging2}
 \begin{tabular}{  l l l l l  } 
  \multirow{2}{3cm}{\textbf{approach}} & \multirow{2}{3cm}{\textbf{intended answer set}} & \multirow{2}{3cm}{\textbf{error types}} & \multirow{2}{2.5cm}{\textbf{user interaction}}  \\\\ \\
  \hline
  \multirow{2}{3cm}{\spock\ transformation 1} & \multirow{2}{3cm}{possible but not required (automatically generated)} & \multirow{2}{3cm}{unsatisfied rule, unsupported atom, unfounded atom} &  possible \\ \\ \\ \\
  \hline 
  \multirow{2}{3cm}{\spock\ transformation 2} & \multirow{2}{3cm}{possible but not required (automatically generated)} & \multirow{2}{3cm}{unsatisfied rule/constraint, unsupported atom, unfounded atom} & possible \\ \\ \\ \\
  \hline
  \ouroboros & required & \multirow{2}{3cm}{unsatisfied rule/constraint, unfounded atom} &  \multirow{2}{2.5cm}{required for intended answer set} \\ \\ \\
  \hline
  interactive \spock & \multirow{2}{3cm}{possible but not required} & \multirow{2}{3cm}{unsatisfied rule/constraint, unsupported atom, unfounded atom} & required \\ \\ \\ \\
  \hline
  \dwasp & \multirow{2}{3cm}{possible but not required} & \multirow{2}{3cm}{minimal unsatisfiable core} & required \\ \\ 
  \hline
  \stepping & \multirow{2}{3cm}{not required but (indirectly) possible} & \multirow{2}{3cm}{unsatisfiability of rules, conflicting truth value of atoms} & required \\ \\ \\
  \hline
 \end{tabular}
 \end{table}



 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsubsection{Knowledge Representation versus Programming}
 As discussed by \citeNS{Cabalar2011}, ASP is seen as a pure knowledge representation and reasoning formalism by some and as a programming language by others.
 It is therefore not surprising that explanation and debugging approaches reflect this difference.
 Seeing ASP as a knowledge representation formalism, a user represents knowledge in terms of a logic program and uses the answer set semantics to find out which conclusions can be drawn from this knowledge.
 The user may also represent a problematic situation and compute answer sets to find a solution to the problem.
 Especially in the latter of these two cases, the user most likely has no idea what the solution may be, in other words, there is no answer set intended by the user.
 On the other hand, if ASP is seen as a programming language, the user may well have an idea of what the solution, i.e. the answer sets, should look like.
 
 Taking these considerations into account, the \spock\ approach (Section~\ref{sec:debugging:spock}) may be more suitable for knowledge representation applications, as it does not require the user to specify an intended answer set.
 Sets of literals are generated automatically as potential answer sets, which are then justified as to why they are not actual answer sets.
 Similarly, the \stepping\ approach (Section~\ref{sec:debugging:stepping}) does not require the user to have an answer set in mind as applicable rules are automatically determined and the user can then freely choose which one to use.
 However, both approaches allow the user to guide the explanation towards specific literals that may be expected in an answer set.
 
 The interactive debugging approaches (Sections~\ref{sec:debugging:interactive} and~\ref{sec:debugging:dwasp}) take a programming language rather than a knowledge representation view on ASP, as they assume that the user has at least some idea as to what an answer set should look like, querying the user about the expected truth value of some literals. The user can certainly choose this truth value at random, making the interactive approaches applicable even if the user has no answer set in mind. However, this does not seem their intended usage. Note also that in order to know the truth value of a literal chosen by the debugging approach, the user essentially has to have a complete answer set in mind as the user does not know upfront which literal will be chosen as a query.
 
 The \ouroboros\ approach (Section~\ref{sec:debugging:ouroboros}) is clearly on the programming language end of the spectrum as it requires the user to specify a complete intended answer set.
 The user could of course choose an ``intended'' answer set at random, but, again, this does not seem the usage envisaged by this approach.
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsubsection{Error Classification}
 As in the case of justifications for consistent logic programs, the debugging approaches also differ regarding the elements used for explaining the inconsistency.
 More precisely, they identify different types of ``errors'' causing a set of literals to not be an answer set.
 Broadly speaking, two different ideas towards errors can be distinguished: the classification of errors into different classes or the reduction of all errors two one ``class''.
 
  \dwasp\ and the \stepping\ approach do not use any named error classes, thus following the latter idea.
  In \dwasp\ errors are sets of rules that, when blocked, make the program consistent.
  However, there is no further explanation as to \emph{why} this is the case.
  On the other hand, errors in the \stepping\ approach are only indirectly specified. They are indicated by (partial) truth assignments to literals, which lead to a contradiction.
  Again, there is no further explanation, other than the rule causing the contradiction.
  In contrast, the other debugging approaches reviewed here distinguish different classes of errors.
 
 The approach by \citeNS{Syrjanen2006} (not discussed here in detail) considers odd-length negative dependency cycles and unsatisfied constraints as errors. 
 In fact, in this approach \emph{all} odd-length negative dependency cycles are classified as ``errors''.
 In contrast, \citeNS{SchulzST2015} (not discussed here in detail either) characterise only \emph{specific} odd-length negative dependency cycles as errors, in addition to sets of literals causing contradictory answer sets.
 Interestingly, none of the debugging approaches reviewed here has an odd-length negative dependency cycle error class.
 This was already discussed for the \spock\ system in Section~\ref{sec:debugging:spock}.
 Consequently, the interactive debugging approach based on \spock\ does not explicitly point out such cycles either, and nor does the \ouroboros\ system, as it implements a subset of the error classes of \spock.

 The \spock\ system and the two approaches based on it (interactive debugging and \ouroboros) use mostly the same classes of errors.
 As previously explained, these are violations of the definition of answer sets by 
 \citeNS{LinZ2004} and \citeNS{Lee2005} (see Definition~\ref{def:answerSet_LinZ_Lee} on page~\pageref{def:answerSet_LinZ_Lee}), namely
 unsatisfied rules, unsupported atoms, and unfounded atoms.
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsubsection{Large and Real-World Logic Programs}
 We already hinted at the fact that the different debugging approaches require various levels of user interaction to obtain an explanation.
 In particular, some approaches require the user to specify an intended answer set before starting the debugging process, especially the \ouroboros\ system.
 This can be difficult if faced with a large logic program, potentially comprising hundreds of atoms.
 Furthermore, using the \stepping\ approach, the user has to step through every single applicable rule, unless being sure that some rules are not problematic for sure, in which case the jumping feature can be used.
% Assuming that the user does not have any idea why the logic program is inconsistent, thus ruling out jumping, the stepping approach can be  for large logic programs.
\CHANGED
Assuming that the user does not have any idea why the logic program is inconsistent, thus ruling out jumping, the stepping approach can take a long time and also be prone to errors for large logic programs.%
\END

 In contrast, for approaches requiring only little user interaction, first and foremost the \spock\ system, the amount of
interaction does not increase when dealing with large logic programs.
 However, it is worth noting that the more literals occur in a program, the more explanations are computed by \spock, namely one for each potential answer set. 
 The user interaction is thus implicitly required after explanations are computed, since the user then has to decide which explanations to take into account.
 It follows, that, just like the \ouroboros\ and \stepping\ approaches, using spock with large logic programs may
\CHANGED
take a long time.
Furthermore, spotting the errors in a large amount of explanations may be difficult for the user.
\END
 
The two interactive approaches (the one based on \spock\ and the \dwasp\ system) may 
\CHANGED
be ones that require least user interaction
\END when handling large logic programs.
This is because queries are determined in such a way that the user's answer provides maximal information gain. Consequently, the total number of queries generated is as small as possible.
From a user's point of view, answering a query on the expected truth value of a single literal may furthermore be easier than specifying the truth value of all literals at once or choosing a meaningful explanation from all the ones generated.
 
 When using ASP in practice, logic programs often include additional language constructs , make use of variables, and are seldom limited to normal rules.
 These are important consideration when choosing a debugging approach. 
 Currently, \ouroboros\ and the \stepping\ approach are the only ones to handle both negation-as-failure and explicit negation, variables, and additional language constructs, where the \stepping\ approach supports more constructs than \ouroboros.
 \dwasp\ supports variables, but to the best of our knowledge no explicit negation or additional language constructs. Nevertheless, is to be assumed that these will be supported in the future since \dwasp\ is implemented in terms of the ASP solver \wasp, which is able to handle these.
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\changed{\section{Related Work}}
\label{sec:related}

\CHANGED
Historically, the idea of justifications can be traced back to~\cite{Shapiro1983} and~\cite{sterling1986explanation} where they have been used as a means for identifying bugs in programs.
Later, \citeN{Lloyd1987} introduced the notions of uncovered atoms and incorrect rules under the completion semantics~\cite{clark1978negation} while \citeN{sterling1989explaining} explained Prolog expert systems using a meta-intepreted.
An important notion for understanding errors in ASP is the concept of supported set, which
was introduced in~\cite{Pereira1991ContradictionRW} and further elaborate in~\cite{PEREIRA1993}.
Another important concept is the  notion of assumptions, which was introduced for truth maintenance systems in~\cite{DEKLEER1986} and developed for logic programming in~\cite{pereira1993debugging}.
\citeN{Specht93} presented one of the first techniques to compute complete proof trees
for bottom-up evaluation of database systems by means of a program transformation.
Further techniques for computing justifications/explanations for Prolog by means of meta-interpreters or program transformations can be found in~\cite{sterling1994art} and~\cite{bratko2001prolog}.



Regarding justifications in ASP, \citeNS{BrainV2005} was one of the first works in tackle this issue by presenting two algorithms for producing natural language explanations as to why a (set of) literal(s) is or is not part of an answer set. 
In the first case, applicable rules are provided as explanation, whereas in the second case contradictions (concerning the truth values of atoms) are pointed out.
Off-line justifications (Section~\ref{sec:offline}, \citeNP{PontelliS2006}) presented a method to compute complete graph justifications expressing why an atoms was or was not in a particular answer set.
As already mentioned, this approach can be traced back to tabled justifications for Prolog~\cite{roychoudhuryRR00,PemmasaniGDRR03}.
\citeNS{PerriRTCV2007} integrate an explanation and debugging component into the \texttt{DLV} solver. 
The root of causal justifications can be traced back to~\cite{Cabalar2011}
where an extension of the stable semantics with causal proofs was introduced
and~\cite{CabalarF13} where an algebraic characterisation of this semantics was developed.
Argumentation-based answer set justifications \cite{SchulzST2013} are a predecessor of LABAS justifications. 
They share the argumentative flavour of LABAS justifications but use a slightly different way of constructing arguments and justifications.
\citeNS{AlbrechtKK2013} show how explanation graphs, as used in off-line justifications, can be constructed from a graphical representation of logic programs called extended dependency graph.
\citeNS{ErdemO2015} use ASP to construct explanations for biomedical queries.
These explanations have a tree structure expressing derivations of a literal in question and have a close relationship with off-line justifications.
 % \comment{The reviewers may say that we should also properly explain this approach, but for now I don't think we have time to do that.}

%For the DLV solver, an explanation and debugging component has been developed \cite{PerriRTCV2007},
%which the authors do not describe in much detail, making it difficult to compare to the justification and debugging approaches reviewed here.

% \comment{is this really necessary? can we omit it?}
Furthermore, explanation approaches have been developed for knowledge representation paradigms related to~ASP.
For instance, \citeNS{AroraRRSS1993} present explanations for deductive databases and \citeNS{FerrandLT2006} for constraint logic programs and constraint satisfaction problems.

As we saw throughout this survey, many justification approaches construct a graphical explanation.
Graph representations of logic programs have also been extensively studied for other purposes \cite{CostantiniDP2002,CostantiniP2010}.
Graphs can for instance be useful for the computation of answer sets, as is the purpose of attack graphs \cite{DimopoulosT1996}, rule graphs \cite{Dimopoulos1996}, and block graphs \cite{Linke2001}
and their extensions \cite{LinkeS2004,KonczakLS2006}.
Furthermore, \citeNS{Costantini2001} and \citeNS{CostantiniP2011} study desirable properties of graphs representing logic programs and \citeNS{Costantini2006} uses cycle graphs to prove conditions for the existence of answer sets.

Various IDEs for ASP also make use of graphical representations of logic programs or visualise dependencies between literals to help the user understand
a problem represented as a logic program.
For example, for the \texttt{DLV} solver a visual computation tracing feature \cite{CalimeriLRV2009} as well as a dependency graph feature \cite{FebbraroRR2011} have been developed.
Furthermore, the \texttt{VIDEAS} system \cite{OetschPSTZ2011} uses entity relationship graphs of logic programs for model-driven engineering in ASP and, in the `Visual ASP' system \cite{FebbraroRR2010}, the user can draw a graph, which is then translated into a logic program.
\END

